Metapath- and Entity-aware Graph Neural Network for Recommendation

In graph neural networks (GNNs), message passing iteratively aggregates nodes' information from their direct neighbors while neglecting the sequential nature of multi-hop node connections. Such sequential node connections e.g., metapaths, capture critical insights for downstream tasks. Concretely, in recommender systems (RSs), disregarding these insights leads to inadequate distillation of collaborative signals. In this paper, we employ collaborative subgraphs (CSGs) and metapaths to form metapath-aware subgraphs, which explicitly capture sequential semantics in graph structures. We propose meta\textbf{P}ath and \textbf{E}ntity-\textbf{A}ware \textbf{G}raph \textbf{N}eural \textbf{N}etwork (PEAGNN), which trains multilayer GNNs to perform metapath-aware information aggregation on such subgraphs. This aggregated information from different metapaths is then fused using attention mechanism. Finally, PEAGNN gives us the representations for node and subgraph, which can be used to train MLP for predicting score for target user-item pairs. To leverage the local structure of CSGs, we present entity-awareness that acts as a contrastive regularizer on node embedding. Moreover, PEAGNN can be combined with prominent layers such as GAT, GCN and GraphSage. Our empirical evaluation shows that our proposed technique outperforms competitive baselines on several datasets for recommendation tasks. Further analysis demonstrates that PEAGNN also learns meaningful metapath combinations from a given set of metapaths.

==> tex/taskformulation.tex <==
% \begin{figure}[!htb]
%   \begin{minipage}{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, left]{figs/HIN.png}
%      \label{fig:HIN}
%      \caption{HIN toy example}\label{Fig:Data1}
%   \end{minipage}\hfill
%   \begin{minipage}[r]{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, valign=t]{figs/schema.png}
%      \label{fig:schema}
%      \caption{HIN schema}
%   \end{minipage}
%   \begin{minipage}[r]{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth, valign=d]{figs/metapaths.png}
%      \label{fig:metapaths}
%      \caption{Metapaths}
%   \end{minipage}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\textwidth,height=4cm]{figs/Intro_1.jpg}
%   \caption{A heterogeneous movie recommendation graph: }
%   \label{fig:HIN}
% \end{figure}
\section{Preliminaries}


% In this section, we start with the definitions of 
% basic concepts used in our models. We then discuss 
% the recommendation task description for
% using collaborative subgraphs 
% as input.
% \subsection{Heterogeneous Information 
% Network and Metapath}
In recommendation tasks, we typically have user-item 
interaction history e.g., purchases and clicks as input.
Those interactions as well as their features can be naturally represented in the setting of a \textbf{Heterogeneous  Information Network} (HIN) \cite{sun2012mining}. A HIN is defined as a graph $G = (V,E)$ with a network schema. 
% A \textbf{Metapath} \cite{sun2011pathsim} is a relation
% sequence composed of several 
% node  and edge types. It encapsulates the 
% structural and semantic relation between connected objects.
%\begin{figure}
%   \begin{minipage}[b]{0.45\textwidth}
%     \centering
%     \subcaptionbox{HIN toy example}{\includegraphics[width=\textwidth]{figs/HIN.png}}
%   \end{minipage}%
% %   \hfill
% %     \begin{minipage}[b]{0.32\textwidth}
% %     \centering
% %     \subcaptionbox{HIN schema}{\includegraphics[width=\textwidth]{figs/schema.png}}
% %   \end{minipage}%
% \hspace{0.1\textwidth}
%   \begin{minipage}[b]{0.45\textwidth}
%     \centering
%         \subcaptionbox{HIN schema}{\includegraphics[width=\textwidth]{figs/schema.png}}
%         \subcaptionbox{Metapaths}{\includegraphics[width=\textwidth]{figs/metapaths.png}}
%   \end{minipage}
% \setlength{\belowcaptionskip}{-8pt}   
%   \caption{An example of heterogeneous information network, its schema and two given metapaths.}
%   \label{fig:example}
% \end{figure}

% The network schema reveals the meta structure of a HIN such as node 
% types $T_v$ and edge types $T_e$, where $|T_v|+|T_e|>2$. 
% A \textbf{Metapath} \cite{sun2011pathsim} is a relation
% sequence composed of several 
% node  and edge types. It encapsulates the 
% structural and semantic relation between connected objects.
% Figures \ref{fig:example}(a)(b) shows a toy example of a HIN for a 
% recommendation task with its network schema. 
% As shown in Fig. \ref{fig:example}(a),
% % the left subfigure, 
% the HIN contains multiple node types (\emph{user}, \emph{gender},
% \emph{movies} etc.) and interaction types (\emph{watches}, \emph{asGender}). 
% Each metapath in 
% Fig. \ref{fig:example}(c)
% encodes unique semantics e.g., the 
% \emph{user}-\emph{gender}-\emph{user} (U-G-U) metapath 
% reveals the shared interest of the same gender, while 
% the \emph{user}-\emph{movie}-\emph{user} (U-M-U)
% metapath indicates the common movie watched by two users. 
% Umer: maybe move this line to actual methodology section
% In this paper, we focus on metapaths ending up with either a user or item node for better distillation of collaborative signals. 

% \subsection{Collaborative Subgraph (CSG)}
A \textbf{Collaborative Subgraph (CSG)} is an $h$-hop undirected enclosing 
subgraph around one user-item pair. 
Given the interaction history and content information 
of a recommendation task, 
the CSG of a user-item pair 
$(u, i)$ is induced from the HIN of the 
recommendation task by nodes $u$, $i$ and their feature entity 
nodes within $h$ hops. Such local subgraphs contain rich 
semantic and collective pattern information of user-item interactions. 
A major difference between our CSGs and the subgraphs proposed by Zhang et al. 
\cite{zhang2019inductive} is that their subgraphs neglect side information by excluding all feature entity nodes.
% \paragraph{Message Passing in Graph Neural Networks (GNNs)} 
% The forward propagation of message passing mechanism in GNNs consists of two phases, a message passing phase and a readout phase. During the message passing phase, vertices in the graph are updated with respect to a message function $Message_t$ and a node update functions $Update_t$, where $t$ denotes the $t$th propagation. During the message passing phase, the update of the hidden state of node $v$ in the graph is written as:
% % \begin{equation}
% \begin{align}%{l}
%     m_v^{t+1} &= \sum_{n\in\mathcal{N}(v)}Message_t(h_v^t, h_n^t, e_{v, n}),\\
%     h_v^{t+1}&=Update_t(h_v^t, m_v^{t+1}),
% \end{align}
% % \end{equation}
% where $m_v^{t+1}$, $\mathcal{N}(v)$ denotes the aggregated message for node $v$ at step $t$ and the neighbours of the node $v$. In the readout phase, the representation for the whole graph should be extracted using a readout function $Readout$ as following:
% \begin{equation}
% \begin{array}{l}
%     h_G = Readout(\{h_v | v \in G\}, G).
% \end{array}
% \end{equation}
% In this paper, we aim to learn a differentiable mapping , which is composed of a message function $Message_t$ and a node update function $Update_t$ in an end-to-end manner.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/framework.png}
      \vspace{-3mm}
    \setlength{\belowcaptionskip}{-8pt}   
    \caption{Illustration of the proposed PEAGNN model on the MovieLens dataset. Subfigure (1) shows the metapath-aware subgraphs generated from a CSG with the given user- and item metapaths. Subfigures (2), (3) and (4) illustrate the metapath-aware information aggregation and fusion workflow of the PEAGNN model. For simplicity, we have only adopted $2$-hop metapaths.}
    \label{fig:framework}
\end{figure*}

\subsection{Task description}
In recommendation tasks, we typically have user-item interaction history as input.
Those interactions as well as their features can be naturally represented in the setting of a \textbf{Heterogeneous  Information Network} (HIN) \cite{sun2012mining}. 
HINs provide a unified framework of representing the relations between user-item interactions and side information with heterogeneous graph structures.
We formulate the recommendation task as follows:
\begin{itemize}[noitemsep]
    \item \textbf{Input} A HIN that includes all 
    user-item historical interactions as well as 
    their feature entity nodes and the initial node 
    embeddings $\mathbf{E}$.
    \item \textbf{Output} Learned heterogeneous node 
    embedding $\mathbf{E}^{\prime}$, a graph encoder \\
    $f_{PEAGNN}(\cdot, \cdot)$ which extracts the graph-level 
    representations from given CSGs
    and a prediction model $f_{\bm{\theta}}(\cdot)$, 
    where $\bm{\theta}$ is a trainable parameter. 
     $f_{\bm{\theta}}(\cdot)$ maps the CSG, whose center is a user-item pair 
    $(u, i)$, to a scalar matching score that the user 
    $u$ would interact with the item $i$.
\end{itemize}

% \paragraph{Metapaths} Given a HIN $G = (V,E, \Psi, \Phi)$, 
% a metapath $M$ is defined as a sequence of node and 
% edge types $(T_{V, 1}, T_{E, 1}, ..., 
% T_{E, n-1}, T_{V, n}, T_{E, n}, ..., 
% T_{E, m-1}, T_{V, m})$ with the abbreviation 
% $T_{V, 1}...T_{V, n}...T_{V, m}$, 
% which denotes a compositional relation $T_{M} = 
% T_{E, 1}\circ...\circ T_{E, n}\circ...\circ T_{E, m}$ 
% connecting nodes $T_{V, 1}$ and $T_{V, m}$, 
% where $\circ$ is the composition operator on relations. 
% Note, for better capturing user preference in recommender 
% system, we only consider the metapath ending up with user 
% node in this paper.

% Two nodes of HINs connected by a metapath are \emph{metapath-guided neighbors}, 
% which was first introduced in item-based Collaborative Filtering [ReF]. 
% For instance, in Figure \ref{HIN} two users can be
% connected via multiple metapaths, e.g., “User-Gender-User”
% (UGU) and “User-Movie-User” (UMU). Each metapath encodes 
% unique semantics e.g., the UGU metapath reveals 
% the shared interest of the same gender, while the UMU metapath 
% indicates the co-watch relations.

% \paragraph{Metapath-based User Subgraphs} Given a metapath $M$ ending up with user node $\{v|v\in V, \Psi(v)=user\}$, a metapath-based user subgraph associated with the metapath $M$ is a user-centered graph, where a center user node $v_{u}$ is connected with all its \emph{metapath-guided neighbors} via the given metapath $M$.

% In a HIN , we typically represent the historical interactions between user and items (e.g., purchases and clicks) as inteaction link between user and items. Here we represent interaction data as a user-item bipartite
% graph G1, which is defined as $\{(u,y_{ui},i)|u \in U,i \in I)\}$, where U
% and I separately denote the user and item sets, and a link yui = 1
% indicates that there is an observed interaction between user u and
% item i; otherwise yui = 0.

% \paragraph{High-order Connectivity}

